On the (In)Security of LLM App Stores

LLM app stores have seen rapid growth, leading to the proliferation of numerous custom LLM apps. However, this expansion raises security concerns. In this study, we propose a three-layer concern framework to identify the potential security risks of LLM apps, i.e., LLM apps with abusive potential, LLM apps with malicious intent, and LLM apps with exploitable vulnerabilities. Over five months, we collected 786,036 LLM apps from six major app stores: GPT Store, FlowGPT, Poe, Coze, Cici, and Character.AI. Our research integrates static and dynamic analysis, the development of a large-scale toxic word dictionary (i.e., ToxicDict) comprising over 31,783 entries, and automated monitoring tools to identify and mitigate threats. We uncovered that 15,146 apps had misleading descriptions, 1,366 collected sensitive personal information against their privacy policies, and 15,996 generated harmful content such as hate speech, self-harm, extremism, etc. Additionally, we evaluated the potential for LLM apps to facilitate malicious activities, finding that 616 apps could be used for malware generation, phishing, etc. Our findings highlight the urgent need for robust regulatory frameworks and enhanced enforcement mechanisms.

==> Tables/toxicdict_language.tex <==
\begin{table}[h!]
\centering
\caption{Counts of words and their data sources across different languages.}
\resizebox{0.75\linewidth}{!}{
\begin{tabular}{lcl}
\toprule[1.2pt]
\textbf{Language} & \textbf{Count} & \textbf{Data source} \\ \midrule
English    & 4833 & Pol. \& Pub. \& LLM \& Trans. \\ 
Chinese    & 4161 & Pol./Pub./LLM/Trans. \\ 
Japanese   & 3531 & Pub./LLM/Trans. \\ 
Korean     & 3519 & Pub./LLM/Trans. \\ 
Portuguese & 4202 & LLM/Trans. \\ 
Spanish    & 3852 & LLM/Trans. \\ 
German     & 3843 & LLM/Trans. \\ 
French     & 3842 & LLM/Trans. \\ \midrule
\textbf{Total}   & \textbf{31783} & \\ 
\bottomrule[1.2pt]
\end{tabular}}
\label{tab:language_counts}
\end{table}

==> Tables/transformation_rules.tex <==
\begin{table*}[h]
\centering
\caption{Transformation rules for toxic word detection.}
\resizebox{\linewidth}{!}{
\begin{tabular}{lll}
\hline
\textbf{Transformation Rule}  & \textbf{Description} & \textbf{Example}    \\ \hline
Repetitions      & Detecting words with repeated characters & ``baaad'' instead of ``bad'' \\
Replacements     & Identifying common substitutions & ``\$'' for ``s'' \\
Emoji Obfuscation & Recognizing toxic words masked with emojis & ``b--d'' for ``bad'' \\
Insertions       & Handling words with inserted characters & ``b\_a\_d'' \\
Special Characters and Spelling Variations & Capturing words with special characters or alternative spellings & ``b@d'' for ``bad'' \\
Leet Speak       & Detecting leet speak variations & ``b@d'' for ``bad'' \\ \hline
\end{tabular}}
\label{tab:transformation}
\end{table*}
